Leveraging User-Generated Metadata of Online Videos for Cover Song Identification

YouTube is a rich source of cover songs. Since the platform itself is organized in terms of videos rather than songs, the retrieval of covers is not trivial. The field of cover song identification addresses this problem and provides approaches that usually rely on audio content. However, including the user-generated video metadata available on YouTube promises improved identification results. In this paper, we propose a multi-modal approach for cover song identification on online video platforms. We combine the entity resolution models with audio-based approaches using a ranking model. Our findings implicate that leveraging user-generated metadata can stabilize cover song identification performance on YouTube.

==> 2_related.tex <==
\section{Related Work}\label{sec:related}

\definecolor{colshs}{rgb}{.447,.624,.812}
\definecolor{colyt}{rgb}{.788,.129,.118}


\begin{figure*}
  \centering
  \includegraphics[scale=0.3]{figs/shs_yt_em.pdf}
  \caption{Example of the text input for a query item (left) and a candidate item (right) of the same work (``Yesterday'' written by John Lennon and Paul McCartney). The query item is a cover of ``Yesterday'' by Jan \& Dean and the candidate item is a cover by Mary Wells. Colors in the box frames and text indicate the data source: \textcolor{colshs}{blue} stands for \textcolor{colshs}{Secondhandsongs} and \textcolor{colyt}{red} for \textcolor{colyt}{YouTube}.}
  
  \label{fig:text_input}
\end{figure*}

Musical entities have been studied in contexts of named entity recognition \cite{ner_epure2023human, ner_nguyen, porcaro2019recognizing_musical_entities, ner_zhang} and also in in entity resolution (ER). The DeepMatcher dataset collection \cite{deep_em_design_space} includes the music domain dataset iTunes-Amazon. The entities are songs from the correspondent streaming services with string attributes (song title, performer, album title, genre tags, copyright information), the length and the release date. Recent deep learning approaches \cite{Li2020DeepEntity, Yao2022EntityResolution} and the popular machine learning approach Magellan \cite{konda2016magellan} achieve F1 scores above 0.9 for this dataset. In contrast to the OCSI task however, the attributes of both data sources are the same (\eg song title to song title) whereas matching song-specific information with YouTube videos is not (\eg song title to video title). 




%Agrawal and Sureka \cite{copyright_infringement_detection} propose a rule-based classification framework for copyright infringement detection. The two stage approach first determines the relevance of YouTube videos with respect to musical works before classifying whether the video is an original or copyright infringement. Another multi-modal approach by Smith, Hamasaki and Goto \cite{classifying_derivative_works} considers video, audio and text features to predict classes of cover versions (\eg karaoke, live performance). The authors use Latent Dirichlet Allocation to learn topics of version types. Using the learned topics as textual features was the most effective feature for the detection of the cover version class.

%In the following, we explain our procedure to leverage user-generated metadata on YouTube for OCSI.

%Musical entities are also studied in entity recognition. An approach by Porcaro and Saggion \cite{porcaro2019recognizing_musical_entities} present an named entity recognition approach to detect musical entities such as titles of symphonies or composers in tweets. Their approach is based on a word embeddings and BiLSTMs-CRF. 



%Abrassart and Doras \cite{what_if_two_musical_versions} combine melodic, harmonic, rhythmic and lyrical features an late-fusion ensemble for the CSI task. Their approach outperforms other audio-based SOTA approaches such as \cite{du2021bytecover, Du2022bytecover2} with lyrics and harmony being the most discriminative features.



%\cite{multimodal_deep_learning_genre_classification}

%\cite{music_libraries_on_youtube} 




%\cite{du2021bytecover}
%\cite{hu2022lyracnet}
%\cite{yu2020cqtnet}

